Evaluating the Zero-shot Robustness of Instruction-tuned Language Models

Instruction fine-tuning has recently emerged as a promising approach for improving the zero-shot capabilities of Large Language Models (LLMs) on new tasks. This technique has shown particular strength in improving the performance of modestly sized LLMs, sometimes inducing performance competitive with much larger model variants. In this paper we ask two questions: (1) How sensitive are instruction-tuned models to the particular phrasings of instructions, and, (2) How can we make them more robust to such natural language variation? To answer the former, we collect a set of 319 instructions manually written by NLP practitioners for over 80 unique tasks included in widely used benchmarks, and we evaluate the variance and average performance of these instructions as compared to instruction phrasings observed during instruction fine-tuning. We find that using novel (unobserved) but appropriate instruction phrasings consistently degrades model performance, sometimes substantially so. Further, such natural instructions yield a wide variance in downstream performance, despite their semantic equivalence. Put another way, instruction-tuned models are not especially robust to instruction re-phrasings. We propose a simple method to mitigate this issue by introducing ``soft prompt'' embedding parameters and optimizing these to maximize the similarity between representations of semantically equivalent instructions. We show that this method consistently improves the robustness of instruction-tuned models.

==> sections/03_instruction_robustness.tex <==


\section{How Robust are Instruction-tuned LLMs?}

%The surge of downstream applications has raised awareness of the other important aspects of instruction-tuned language models besides best performances. 
Instruction-tuning has shown promise in improving zero-shot performance of LLMs, especially for comparatively small models \cite{alpaca,longpre2023flan,sanh2021multitask}.
Indeed, careful instruction-tuning of ``smaller'' models like T5-XL (3B parameters) can result in zero-shot performance that is competitive with---or even better than---much larger models \cite{longpre2023flan}.
Realizing such functionality with modestly sized models is an important and timely research goal, and instruction-tuning has emerged as a promising means to this end. 

The promise of such models lies in their ability to perform novel tasks specified via natural language instructions. 
It is therefore important that models are robust to variations in instruction phrasings: Semantically equivalent instructions should yield comparable results.
However, we find that instruction-tuned LLMs are (sometimes very) sensitive to changes in phrasings, with novel instructions (i.e., instructions unobserved in training) leading to substantially degraded performance. 


\begin{figure}[h]
    \centering
    \includegraphics[scale=0.5]{images/robustness_cropped.pdf}
    \caption{In this example, the observed instruction is the \textit{Task 1286} in NIV2 \cite{wang2022benchmarking} using \textit{Template 6}, whereas the unobserved is written by NLP practitioner specifically for MMLU \cite{hendrycks2020measuring}}
    \label{fig:my_label}
\end{figure}
%For a specific task, a \textbf{robust} model, after instruction-tuning, ought to perform equally well when given two semantically equivalent instructions







